Variable-lag Granger Causality and Transfer Entropy for Time Series Analysis

Granger causality is a fundamental technique for causal inference in time series data, commonly used in the social and biological sciences. Typical operationalizations of Granger causality make a strong assumption that every time point of the effect time series is influenced by a combination of other time series with a fixed time delay. The assumption of fixed time delay also exists in Transfer Entropy, which is considered to be a non-linear version of Granger causality. However, the assumption of the fixed time delay does not hold in many applications, such as collective behavior, financial markets, and many natural phenomena. To address this issue, we develop Variable-lag Granger causality and Variable-lag Transfer Entropy, generalizations of both Granger causality and Transfer Entropy that relax the assumption of the fixed time delay and allow causes to influence effects with arbitrary time delays. In addition, we propose methods for inferring both variable-lag Granger causality and Transfer Entropy relations. In our approaches, we utilize an optimal warping path of Dynamic Time Warping (DTW) to infer variable-lag causal relations. We demonstrate our approaches on an application for studying coordinated collective behavior and other real-world casual-inference datasets and show that our proposed approaches perform better than several existing methods in both simulated and real-world datasets. Our approaches can be applied in any domain of time series analysis. The software of this work is available in the R-CRAN package: VLTimeCausality.

==> 05-method.old.tex <==
\section{VL-Granger and Transfer Entropy Causality Inference}

\subsection{VL-Granger Causality Inference}
Given a target time series $Y$, a candidate causing time series $X$, a threshold $\gamma$, a significance level $\alpha$, and the max lag $\delta_{max}$, our framework evaluates whether $X$ VL-Granger causes $Y$ (with a variable lag), $X$ Granger causes $Y$ (with a fixed lag) or no conclusion of causation between $X$ and $Y$. 

 In Algorithm~\ref{algo:MainFunc} line 1-2,  we have a fix-lag parameter $FixLag$ that controls whether we choose to compute the normal Granger causality ($FixLag=true$) or VL-Granger causality ($FixLag=false$). We present the high level logic of the algorithm. However, the actual implementation is more efficient by removing the redundancies of the presented logic.

 First, we compute Granger causality (line 1 in  Algorithm~\ref{algo:MainFunc}). The flag $GrangerResult=true$ if $X$ Granger-causes $Y$, otherwise $GrangerResult=false$. Second, we  compute VL-Granger causality (line 2 in  Algorithm~\ref{algo:MainFunc}). The flag $VLGrangerResult=true$ if $X$ VL-Granger-causes $Y$, otherwise $VLGrangerResult=false$. 
 
  Based on the work in~\cite{atukeren2010relationship}, we use the Bayesian Information Criteria  (BIC) to compare the residual of regressing $Y$ on $Y$ past information, $r_Y$, with the residual of regressing $Y$ on $Y$ and $X$ past information $r_{YX}$. We use $v_1 \ll v_2$ to represent that $v_1$ is less than $v_2$ with statistical significance by using some statistical test(s). If $BIC(r_Y)\ll BIC(r_{YX})$, then we conclude that the prediction of  $Y$  using $Y,X$ past information is better than the prediction of  $Y$  using $Y$ past information alone. For this work, to determine $BIC(r_Y)\ll BIC(r_{YX})$, we use \textit{Bayesian Information Criterion difference ratio} (see Section~\ref{sec:BICDiffratio}).
  
Using the results of both  $GrangerResult$ and $VLGrangerResult$, we proceed to report the conclusion of causal relation between $X$ and $Y$ w.r.t.  the following four conditions.
 
 \squishlist
\item {\bf If both $GrangerResult$ and $VLGrangerResult$ are true}, then we compare the residual of variable-lag regression $r_{DTW}$ with both$r_Y$ and $r_{YX}$. If $BIC(r_{DTW}) < min(BIC(r_{YX}),BIC(r_{Y}) )$, then we conclude that $X$ causes $Y$ with variable lags, otherwise, $X$ causes $Y$ with a fix lag (line 4 in  Algorithm~\ref{algo:MainFunc}).
\item {\bf If $GrangerResult$ is true but $VLGrangerResult$ is false}, then we conclude that $X$ causes $Y$ with a fix lag (line 5 in Algorithm~\ref{algo:MainFunc}).
\item {\bf If $GrangerResult$ is false but $VLGrangerResult$ is true}, then we conclude that $X$ causes $Y$ with variable lags (line 6 in Algorithm~\ref{algo:MainFunc}).

\item {\bf If both $GrangerResult$ and $VLGrangerResult$ are false}, then we cannot conclude whether $X$ causes $Y$ (line 7 in Algorithm~\ref{algo:MainFunc}).
\squishend

\setlength{\intextsep}{0pt}
\IncMargin{1em}
\begin{algorithm2e}
\caption{Time-lag test function}
\label{algo:MainFunc}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{ $X,Y$, $\sigma$, $\alpha$, $\delta_{max}$ }
\Output{$XGrangerCausesY$}
\begin{small}
\SetAlgoLined
\nl ($GrangerResult$,$r_{Y},r_{YX}$)=VLGrangerFunc($X,Y$, $\sigma$, $\alpha$, $\delta_{max}$, $FixLag = true$)\;
\nl ($VLGrangerResult$,$r_{Y},r_{DTW}$)= VLGrangerFunc($X,Y$, $\sigma$, $\alpha$, $\delta_{max}$, $FixLag = false$)\;
\nl \uIf{$GrangerResult=true$ }
{
                 \uIf{$VLGrangerResult=true$}
                {
                
               \nl   \uIf{$BIC(r_{DTW}) \ll min(BIC(r_{YX}),BIC(r_{Y}) )$}
                {
                $XGrangerCausesY$ = TRUE-VARIABLE\; %$X$ causes $ Y$ with variable lags \;
                }
                 \Else{
                $XGrangerCausesY$ = TRUE-FIXED\; %$X$ causes $ Y$ with a fixed lag\;
                }              
                
                }
                \Else{
                \nl  $XGrangerCausesY$ = TRUE-FIXED\; %$X$ causes $ Y$ with a fixed lag\;
                }
} 
 \Else{
  				\uIf{$VLGrangerResult=true$}
                {
                 \nl  $XGrangerCausesY$ = TRUE-VARIABLE\; %$X$ causes $ Y$ with variable lags\;
                }
                 \Else{
                \nl  $XGrangerCausesY$ = NONE\; %We cannot conclude whether $X$ causes $ Y$\;
                }
}
\nl return $XGrangerCausesY$\;
\end{small}
\end{algorithm2e}\DecMargin{1em}

Note that we assume the maximum lag value $\delta_{\max}$ is given as an input, as it is for all definitions of Granger causality. For practical purposes, a value of a large fraction ({\em e.g., } half) of the length of the time series can be used. However, there is, of course, a computational trade-off between the magnitude of $\delta_{\max}$ and the time it takes to compute Granger causality.

\subsection{VL-Granger causality operationalization}
Next, we describe the details of the VL-Granger function used in Algorithm~\ref{algo:MainFunc}: line 1-2. Given two time series $X$ and $Y$, a threshold $\gamma$, a significance level $\alpha$, the maximum possible lag $\delta_{max}$, and whether we want to check for variable or fixed lag $FixLag$, Algorithm~\ref{algo:VLGrangerCalFunc} reports whether $X$ causes $Y$ by setting $GrangerResult$ to true or false, and by reporting on two residuals  $r_{Y}$ and $r_{YX}$.

First, we compute the residual $r_Y$ of regressing of $Y$ on $Y$'s information in the past (line 1). Then, we regress $Y(t)$ on $Y$ and $X$ past information to compute the residual $r_{YX}$ (line 2). If $BIC(r_{YX}) \ll BIC(r_{Y})$, then $X$ Granger-causes $Y$ and we set $GrangerResult=true$ (line 7). 
If $FixLag$ is true, then we report the result of typical Granger causality. Otherwise, we consider VL-Granger causality (lines 3-5) by computing the emulation relation between $X^{DTW}$ and $Y$ where $X^{DTW}$ is a version of $X$ that is reconstructed through DTW and is most similar to $Y$, captured by $DTWReconstructionFunction(X,Y)$ which we explain in Section~\ref{sec:DTWRecont}. 

Afterwards, we do the regression of $Y$ on $X^{DTW}$'s past information to compute  residual $r_{DTW}$ (line 4). Finally, we check whether $BIC(r_{DTW}) \ll BIC(r_{Y})$ (line 6-9) (see Section~\ref{sec:BICDiffratio}). If so, $X$ VL-Granger-cause $Y$.  In the next section, we describe the details of how to construct $X^{DTW}$ and how to estimate the emulation similarity value $simValue$.

\setlength{\intextsep}{0pt}
\IncMargin{1em}
\begin{algorithm2e}
\caption{VLGrangerFunc}
\label{algo:VLGrangerCalFunc}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$X,Y$, $\delta_{max}$, $\alpha$, $\gamma$, $FixLag$ }
\Output{ $GrangerResult$,$r_{Y},r_{YX}$}
\begin{small}
\SetAlgoLined
 \nl Regress $Y(t)$ on $Y(t-\delta_{max}),\dots, Y(t-1)$, then compute the residual $r_{Y}(t)$\;
 
  \uIf{$FixLag$ is true}{
   \nl Regress $Y(t)$ on $Y(t-\delta_{max}),\dots, Y(t-1)$ and $X(t-\delta_{max}),\dots, X(t-1)$, then compute the residual  $r_{YX}(t)$\;
  }
 \Else{
 \nl $X^{DTW}$,$simValue$ = DTWReconstructionFunction($X,Y$) \;
 \nl  Regress $Y(t)$ on $Y(t-\delta_{max}),\dots, Y(t-1)$ and $X^{DTW}(t-\delta_{max}),\dots, X^{DTW}(t-1)$, then compute the residual  $r_{DTW}$\;
 \nl $r_{YX}=r_{DTW}$\;
 } %== end else
 
 \nl \uIf{$BIC_1(r_{YX}) \ll BIC_0(r_{Y})$  } 
{
\nl $GrangerResult=true$
}
\nl \Else{
\nl $GrangerResult=false$ \;}
\nl return $GrangerResult$,$r_{Y},r_{YX} $\;
\end{small}
\end{algorithm2e}\DecMargin{1em}


\subsection{Dynamic Time Warping for inferring VL-Granger causality.}
\label{sec:DTWRecont}

In this work, we propose to use Dynamic Time Warping (DTW)~\cite{sakoe1978dynamic}, which is a standard distance measure between two time series.  DTW calculates the distance between two time series by aligning sufficiently similar patterns between two time series, while allowing for local stretching (see Figure~\ref{fig:LinearVSArbLag}). Thus, it is particularly well suited for calculating the variable lag alignment. 

Given time series $X$ and $Y$, Algorithm~\ref{algo:DTWReFunc} reports reconstructed time series $X^{DTW}$ based on $X$ that is most similar to $Y$, as well as the emulation similarity $simValue$ between the two series. 
First, we use $DTW(X,Y)$ to find the optimal alignment sequence $\hat{P}=(\Delta_1,\dots,\Delta_t,\dots)$ between $X$ and $Y$, as defined in Definition~\ref{def:AlignSeq}. Efficient algorithms for computing $DTW(X,Y)$ exist and they can incorporate various kernels between points~\cite{Mueen:2016:EOP:2939672.2945383,sakoe1978dynamic}. Then, we use $\hat{P}$ to construct $X^{DTW}$ where $X^{DTW}(t)=X(t-\Delta_t)$. However, we also use cross-correlation to normalize  $\Delta_t$ since DTW is sensitive to a noise of alignment (Algorithm~\ref{algo:DTWReFunc} line 3-5). 

Afterwards, we use $X^{DTW}$ to predict $Y$ instead of using only $X$ information in the past in order to infer a VL-Granger causal relation in Definition~\ref{def:ArbCausalR}. The benefit of using DTW is that it can match time points of $Y$ and $X$ with non-fixed lags (see Figure~\ref{fig:LinearVSArbLag}). Let $\hat{P}=(\Delta_1,\dots,\Delta_t,\dots)$ be the DTW optimal warping path of $X,Y$ such that for any $\Delta_t \in \hat{P}$, $Y(t)$ is most similar to $X(t-\Delta_t)$. 

In addition to finding $X^{DTW}$, $DTWReconstructionFunction$ estimates the emulation similarity $simValue$ between $X,Y$ in line 3. For that, we adopt the measure from~\cite{FLICAtkdd} below: 

% Mention: In our experiments we used Euclidean distance for the kernel but this is general enough that it can capture others as well. In essence, we can only match based on predetermined kernels vs. ones we discover.

\begin{equation}
	\mathrm{s}(\hat{P})=\frac{\sum_{\Delta_t \in \hat{P}}\mathrm{sign}(\Delta_t)}{|\hat{P}|},
	\label{eq:traCorr}
\end{equation}
where $0<\mathrm{s}(\hat{P})\leq 1$ if $X\preceq Y$,  $-1\leq \mathrm{s}(\hat{P})<0$ if $Y\preceq X$, otherwise zero. Since the $\mathrm{sign}(\Delta_t)$ represents whether $Y$ is similar to $X$ in the past ($\mathrm{sign}(\Delta_t) >0$) or  $X$ is similar to $Y$ in the past ($\mathrm{sign}(\Delta_t) <0$), by comparing the sign of $\mathrm{sign}(\Delta_t)$, we can infer whether $Y$ emulates $X$. The function $\mathrm{s}(\hat{P})$ computes the average sign of   $\mathrm{sign}(\Delta_t)$ for the entire time series. If $\mathrm{s}(\hat{P})$ is positive, then, on average, the number of times that $Y$ is similar to $X$ in the past is greater than the number of times that $X$ is similar to some values of $Y$ in the past.  Hence, $\mathrm{s}(\hat{P})$ can be used as a proxy to determine whether $Y$ emulates $X$ or vice versa.  We use \textit{dtw} R package~\cite{giorgino2009computing} for our DTW function.

\setlength{\intextsep}{0pt}
\IncMargin{1em}
\begin{algorithm2e}
\caption{ DTWReconstructionFunction}
\label{algo:DTWReFunc}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{ $X,Y$}
\Output{ $X^{DTW}$, $simValue$}
\begin{small}
\SetAlgoLined
\nl $\hat{P}=(\Delta_1,\dots,\Delta_t,\dots)$ = DTW( $X,Y$) \;
\nl $\hat{P}_0=(\Delta_0,\dots,\Delta_0,\dots)$=CrossCorrelation($X,Y$)\;
\nl \For{ all $t$}{
 \uIf{$DIST(X(t-\Delta_t),Y(t))<DIST(X(t-\Delta_0),Y(t))$}
 {
 \nl set  $X^{DTW}(t-1)=X(t-\Delta_t)$ and $\hat{P}^*(t)=\Delta_t$\;
 }\Else{
 \nl set  $X^{DTW}(t-1)=X(t-\Delta_0)$ and $\hat{P}^*(t)=\Delta_0$ \;
 }
}
\nl        $simValue =\mathrm{s}(\hat{P}^*)$ \;
Return $X^{DTW}$, $simValue$\;
\end{small}
\end{algorithm2e}\DecMargin{1em}

\subsection{Bayesian Information Criterion difference ratio for VL-Granger causality}
\label{sec:BICDiffratio}

Given $RRSS$ is a restricted residual sum of squares from a regression of $Y$ on $Y$ past, and $T$ is a length of time series, the BIC of null model can be defined below. 
\label{sec:BICdiffratio}
\begin{equation}
	BIC_0(r_{Y})=\frac{RRSS(r_{Y})}{T}T^{(\delta_{max}+1)/T},
	\label{eq:BICrest}
\end{equation}

For unrestricted model, given $URSS$ is an unrestricted residual sum of squares from a regression of $Y$ on $Y,X$ past, and $T$ is a length of time series, the BIC of alternative model can be defined below. 
\begin{equation}
	BIC_1(r_{YX})=\frac{URSS(r_{YX})}{T}T^{(2\delta_{max}+1)/T},
	\label{eq:BICunrest}
\end{equation}
We use the \textit{Bayesian Information Criterion difference ratio} as a main criteria to determine whether $X$ Granger-causes $Y$ or determining $BIC_1(r_{YX}) \ll BIC_0(r_{Y})$ in Algorithm~\ref{algo:VLGrangerCalFunc} line 6, which can be defined below:
\begin{equation}
	\mathrm{r}(BIC_0(r_{Y}),BIC_1(r_{YX}))=\frac{BIC_0(r_{Y})-BIC_1(r_{YX})}{BIC_0(r_{Y})}.
	\label{eq:BICdiffRatio}
\end{equation}

The ratio $\mathrm{r}(\cdot,\cdot)$ is within $[-\infty,1]$. The closer $\mathrm{r}(\cdot,\cdot)$  to $1$, the better the performance of alternative model is compared to the null model. We can set the threshold $\gamma\in[0,1]$ to determine whether $X$ Granger-causes $Y$, i.e. $\mathrm{r}(BIC_0(r_{Y}),BIC_1(r_{YX}))\geq \gamma$ implies $X$ Granger-causes $Y$. Other options of determining $X$ Granger-causes $Y$ is to use F-test or the emulation similarity $simValue$.

\subsection{VL-Transfer-Entropy Causality Inference}
\label{sec:VLTEmethod}
Given a target time series $Y$, a candidate causing time series $X$, and the max lag $\delta_{max}$, our framework evaluates whether $X$ causes $Y$ in VL-Transfer-Entropy (with a variable lag), $X$ causes $Y$ in  Transfer-Entropy (with a fixed lag) or no conclusion of causation can be reached between $X$ and $Y$. 

In Algorithm~\ref{algo:TransferEntropyMainFunc} line 1-2,  we have a fixed-lag parameter $FixLag$ that controls whether we choose to compute the normal Transfer-Entropy causality ($FixLag=true$) or VL-Transfer-Entropy causality ($FixLag=false$).  

\setlength{\intextsep}{0pt}
\IncMargin{1em}
\begin{algorithm2e}
\caption{Transfer Entropy Time-lag test function}
\label{algo:TransferEntropyMainFunc}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{ $X,Y$, $\delta_{max}$ }
\Output{$XTransferEntropyCausesY$}
\begin{small}
\SetAlgoLined
\nl ($TransEResult$,$\mathcal{T}_{X\xrightarrow{} Y},\mathcal{T}_{Y\xrightarrow{} X}$)=VLTransferEFunc($X,Y$, $\sigma$, $\alpha$, $\delta_{max}$, $FixLag = true$)\;
\nl ($VLTransEResult$,$\mathcal{T}^\text{VL}_{X\xrightarrow{} Y},\mathcal{T}^\text{VL}_{Y\xrightarrow{} X}$)=VLTransferEFunc($Y,X$, $\sigma$, $\alpha$, $\delta_{max}$, $FixLag = false$)\;
\nl \uIf{$TransEResult=true$ }
{
                 \uIf{$VLTransEResult=true$}
                {
                
               \nl   \uIf{$\mathcal{T}(X,Y)_\textrm{ratio} < \mathcal{T}^\text{VL}(X,Y)_\textrm{ratio}$}
                {
                $XTransferEntropyCausesY$ = TRUE-VARIABLE\; %$X$ causes $ Y$ with variable lags \;
                }
                 \Else{
                $XTransferEntropyCausesY$ = TRUE-FIXED\; %$X$ causes $ Y$ with a fixed lag\;
                }              
                
                }
                \Else{
                \nl  $XTransferEntropyCausesY$ = TRUE-FIXED\; %$X$ causes $ Y$ with a fixed lag\;
                }
} 
 \Else{
  				\uIf{$VLTransEResult=true$}
                {
                 \nl  $XTransferEntropyCausesY$ = TRUE-VARIABLE\; %$X$ causes $ Y$ with variable lags\;
                }
                 \Else{
                \nl  $XTransferEntropyCausesY$ = NONE\; %We cannot conclude whether $X$ causes $ Y$\;
                }
}
\nl return $XTransferEntropyCausesY$\;
\end{small}
\end{algorithm2e}\DecMargin{1em}


First, we compute Transfer Entropy causality (line 1 in  Algorithm~\ref{algo:TransferEntropyMainFunc}). The flag $TransEResult=true$ if $X$ Transfer-Entropy-causes $Y$, otherwise $TransEResult=false$. Second, we  compute VL-Transfer-Entropy causality (line 2 in  Algorithm~\ref{algo:TransferEntropyMainFunc}). The flag $VLTransEResult=true$ if $X$ VL-Transfer-Entropy-causes $Y$, otherwise $VLTransEResult=false$. 
 
 To determine whether $X$ Transfer-Entropy-causes $Y$, we can use the \textit{Transfer Entropy Ratio}.

\begin{equation}
\label{eq:trnsEnpRatio}
    \mathcal{T}(X,Y)_\textrm{ratio} =\frac{\mathcal{T}_{X\xrightarrow{} Y}}{\mathcal{T}_{Y\xrightarrow{} X}} .
\end{equation}

The \textit{VL-Transfer Entropy Ratio} is defined below:

\begin{equation}
\label{eq:VLtrnsEnpRatio}
    \mathcal{T}^\text{VL}(X,Y)_\textrm{ratio} =\frac{\mathcal{T}^\text{VL}_{X\xrightarrow{} Y}}{\mathcal{T}^\text{VL}_{Y\xrightarrow{} X}} .
\end{equation}

$\mathcal{T}(X,Y)_\textrm{ratio}$ greater than $1$ implies that $X$ Transfer-Entropy-causes $Y$. The higher $\mathcal{T}(X,Y)_\textrm{ratio}$, the higher the strength of $X$ causing $Y$. The same is true for $\mathcal{T}^\text{VL}(X,Y)_\textrm{ratio}$.
 
Using the results of both  $TransEResult$ and $VLTransEResult$, we proceed to report the conclusion of causal relation between $X$ and $Y$ w.r.t.  the following four conditions:
 
 \squishlist
\item {\bf If both $TransEResult$ and $VLTransEResult$ are true}, then we compare the $\mathcal{T}(X,Y)_\textrm{ratio}$ with $\mathcal{T}^\text{VL}(X,Y)_\textrm{ratio}$. If $\mathcal{T}(X,Y)_\textrm{ratio} < \mathcal{T}^\text{VL}(X,Y)_\textrm{ratio}$, then we conclude that $X$ causes $Y$ with variable lags, otherwise, $X$ causes $Y$ with a fix lag (line 4 in  Algorithm~\ref{algo:TransferEntropyMainFunc}).
\item {\bf If $TransEResult$ is true but $VLTransEResult$ is false}, then we conclude that $X$ causes $Y$ with a fix lag (line 5 in Algorithm~\ref{algo:TransferEntropyMainFunc}).
\item {\bf If $TransEResult$ is false but $VLTransEResult$ is true}, then we conclude that $X$ causes $Y$ with variable lags (line 6 in Algorithm~\ref{algo:TransferEntropyMainFunc}).

\item {\bf If both $TransEResult$ and $VLTransEResult$ are false}, then we cannot conclude whether $X$ causes $Y$ (line 7 in Algorithm~\ref{algo:TransferEntropyMainFunc}).
\squishend

\subsection{VL-Transfer-Entropy causality operationalization}
Given time series $X,Y$, and the maximum possible lag $\delta_{max}$, and whether we want to check for variable or fixed lag $FixLag$, Algorithm~\ref{algo:VLTransferEFunc} reports whether $X$ causes $Y$ by setting $TransEResult$ to true or false, and by reporting on two transfer entropy values: $\mathcal{T}_{X\xrightarrow{} Y}$ and $\mathcal{T}_{Y\xrightarrow{} X}$.

First, if $FixLag$ is true, then we compute the transfer entropy (line 1) using RTransferEntropy($X,Y$)~\cite{BEHRENDT2019100265}. If $FixLag$ is false, then, we reconstructed $X^{DTW}$ using $DTWReconstructionFunction(X,Y)$ in Section~\ref{sec:DTWRecont} (line 2). We compute the VL-transfer entropy (line 3) using RTransferEntropy($X^{DTW},Y$).

If the ratio $\mathcal{T}(X,Y)_\textrm{ratio}>1$, then $X$ causes $Y$ and we set $TransEResult=true$ (line 5), otherwise, $TransEResult=false$ (line 7). 

\setlength{\intextsep}{0pt}
\IncMargin{1em}
\begin{algorithm2e}
\caption{VLTransferEFunc}
\label{algo:VLTransferEFunc}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$X,Y$, $\delta_{max}$, $FixLag$ }
\Output{ $TransEResult$,$\mathcal{T}_{X\xrightarrow{} Y}$,$\mathcal{T}_{Y\xrightarrow{} X}$}
\begin{small}
\SetAlgoLined
  \uIf{$FixLag$ is true}{
   \nl $\mathcal{T}_{X\xrightarrow{} Y}$,$\mathcal{T}_{Y\xrightarrow{} X}$ = RTransferEntropy($X,Y$)~\cite{BEHRENDT2019100265}\;
  }
 \Else{
 \nl $X^{DTW}$,$simValue$ = DTWReconstructionFunction($X,Y$) \;
 \nl $\mathcal{T}_{X\xrightarrow{} Y}$,$\mathcal{T}_{Y\xrightarrow{} X}$ = RTransferEntropy($X^{DTW},Y$)~\cite{BEHRENDT2019100265}\;
 } %== end else
 
 \nl \uIf{$\mathcal{T}(X,Y)_\textrm{ratio}>1$  } 
{
\nl $TransEResult=true$
}
\nl \Else{
\nl $TransEResult=false$ \;}
\nl return $TransEResult$,$\mathcal{T}_{X\xrightarrow{} Y}$,$\mathcal{T}_{Y\xrightarrow{} X}$\;
\end{small}
\end{algorithm2e}\DecMargin{1em}
